Breaking the Cubic Barrier for All-Pairs Max-Flow: Gomory-Hu Tree in Nearly Quadratic Time

In 1961, Gomory and Hu showed that the All-Pairs Max-Flow problem of computing the max-flow between all $n\choose 2$ pairs of vertices in an undirected graph can be solved using only $n-1$ calls to any (single-pair) max-flow algorithm. Even assuming a linear-time max-flow algorithm, this yields a running time of $O(mn)$, which is $O(n^3)$ when $m = \Theta(n^2)$. While subsequent work has improved this bound for various special graph classes, no subcubic-time algorithm has been obtained in the last 60 years for general graphs. We break this longstanding barrier by giving an $\tilde{O}(n^{2})$-time algorithm on general, weighted graphs. Combined with a popular complexity assumption, we establish a counter-intuitive separation: all-pairs max-flows are strictly easier to compute than all-pairs shortest-paths. Our algorithm produces a cut-equivalent tree, known as the Gomory-Hu tree, from which the max-flow value for any pair can be retrieved in near-constant time. For unweighted graphs, we refine our techniques further to produce a Gomory-Hu tree in the time of a poly-logarithmic number of calls to any max-flow algorithm. This shows an equivalence between the all-pairs and single-pair max-flow problems, and is optimal up to poly-logarithmic factors. Using the recently announced $m^{1+o(1)}$-time max-flow algorithm (Chen et al., March 2022), our Gomory-Hu tree algorithm for unweighted graphs also runs in $m^{1+o(1)}$-time.

==> prelim.tex <==

\section{Preliminaries}


%Let $G=(V,E)$ be an undirected graph with an edge-weight function
%$w\in\mathbb{R}_{>0}^{E}$. If $w(e)=1$ for all $e\in E$, then we
%say $G$ is unweighted. For any edge set $E'\subseteq E$, $w(E')=\sum_{e\in E'}w(e)$
%the total weight of edges in $E'$. For any cut $(S,V\setminus S)$,
%we also refer to a side $S$ of this cut as a cut. The \emph{size
%of cut $S$} is $\delta(S)=w(E(S,V\setminus S))$. 

For any two disjoint
vertex sets $A,B\subset V$, we say that $S$ is an \emph{$(A,B)$-cut}
if $A\subseteq S$ and $B\cap S=\emptyset$ or $B\subseteq S$ and
$A\cap S=\emptyset$. $S$ is an \emph{$(A,B)$-mincut} if it is
an $(A,B)$-cut with minimum size.\amir{I moved everything except for the definitions of $A,B$-cuts to the overview. This definitnon is only needed for isolating cuts, right? maybe we can have it local to section 3?} Let $\lambda(A,B)$ denote the
size of $(A,B)$-mincut. 
%When $A=\{a\}$ and $B=\{b\}$, then $(a,b)$-cut,
%$(a,b)$-mincut, and $\lambda(a,b)$ are defined similarly. 

%Let $U \subseteq V$ be a terminal set of vertices. 
%The \emph{$U$-Steiner connectivity/mincut} is $\lambda(U)=\min_{a,b\in U}\lambda(a,b)$. 
%A tree $T$ is a \emph{$U$-Steiner tree} if $U \subseteq V(T)$. When $U$ is clear
%from the context, we write Steiner instead of $U$-Steiner.
%Let $(A,V\setminus A)$ be a cut and $C$ be the edge set crossing this cut. We say that a tree $T$ \emph{$k$-respects} a cut $(A,V\setminus A)$ (and vice versa) if $E(T)\cap C = k$.



%\begin{definition}[$k$-respecting terminal-spanning tree]
%**TODO [state and move to overview]**
%Let $G=(V,E)$ be an undirected graph on $n$ nodes with terminals $U\subseteq V$. 
%A $k$-respecting terminal-spanning tree $T$ is an unweighted tree on vertex set $U$ such that for any pair $s,t\in U$ there is a minimum $s,t$-cut $C$ in $G$ that cuts only $\leq 4$ edges in $T$, i.e. the cut $C \cap U$ has value $\leq 4$ in $T$. 
%\end{definition}
